DiffPLF: A Conditional Diffusion Model for Probabilistic Forecasting of EV Charging Load

Due to the vast electric vehicle (EV) penetration to distribution grid, charging load forecasting is essential to promote charging station operation and demand-side management.However, the stochastic charging behaviors and associated exogenous factors render future charging load patterns quite volatile and hard to predict. Accordingly, we devise a novel Diffusion model termed DiffPLF for Probabilistic Load Forecasting of EV charging, which can explicitly approximate the predictive load distribution conditioned on historical data and related covariates. Specifically, we leverage a denoising diffusion model, which can progressively convert the Gaussian prior to real time-series data by learning a reversal of the diffusion process. Besides, we couple such diffusion model with a cross-attention-based conditioning mechanism to execute conditional generation for possible charging demand profiles. We also propose a task-informed fine-tuning technique to better adapt DiffPLF to the probabilistic time-series forecasting task and acquire more accurate and reliable predicted intervals. Finally, we conduct multiple experiments to validate the superiority of DiffPLF to predict complex temporal patterns of erratic charging load and carry out controllable generation based on certain covariate. Results demonstrate that we can attain a notable rise of 39.58% and 49.87% on MAE and CRPS respectively compared to the conventional method.

==> proposal.tex <==
\subsection{Problem Formulation}
In this paper, we focus on the problem of day-ahead probabilistic charging load forecasting. Different from the point prediction which aims to determine exact results of the future charging load, probabilistic forecasting is dedicated to model the forecast uncertainties by approximating the conditional distribution of the future outcomes. In \textcolor{red}{To be }specific, given the historical charging load data $\mathbf{x}_{d-1:d-N}$ of $N$ past days, our goal is to procure the distribution over all possible charging load profiles $\mathbf{x}_{d}$ in the next day $d$. Besides, we leverage certain covariates $\mathbf{c}_{d}$ as complementary conditions, which should be known for day $d$ in advance and conducive to elicit more realistic outcomes of $\mathbf{x}_{d}$. Since EV charging behaviors are associated with weather conditions and calendar variables, we employ the weather forecast data $\mathbf{w}_{d}$ and day type $y_{d}$ as additional covariates, i.e., $\mathbf{c}_{d}=[\mathbf{w}_{d},y_{d}]$. Therefore, we aim to accurately estimate the following conditional distribution:
\begin{equation}
\centering
p(\mathbf{x}_{d}|\mathbf{x}_{d-1:d-N},\mathbf{w}_{d},y_{d})
\label{eq:1}
\end{equation}

\textcolor{blue}{Proposal to solve \eqref{eq:1}: }Conditional DDPM + Cross-attention mechanism
In this part, we explore how to further enhance the accuracy and reliability of PI. Furthermore, according to~\cite{9760076}, in terms of a potent probabilistic forecasting model, the expected value of the forecasting outcomes is anticipated to be equal to the true point forecast. In other words, once we utilize the well trained diffusion model to generate a batch of charging load profiles $\mathbf{x}^{gen}_{d}$ at day $d$, the ideal mean value of them should approach the real $\mathbf{x}^{true}_{d}$ as close as possible. In light of this, we have another optimization objective as follows:
\begin{equation}
\centering
min \left \| \mathrm {E}[\mathbf{x}^{gen}_{d}]-\mathbf{x}^{true}_{d} \right \|^{2}
\label{eq:2}
\end{equation}

\textcolor{blue}{Proposal to solve \eqref{eq:2}: }Inspired by the prior class preservation loss proposed in~\cite{Ruiz_2023_CVPR}, we attempt to fine-tune the trained denoising network $\epsilon_{\theta}(\cdot)$ using the following loss function: \textcolor{yellow}{inductive bias, stochastic sampling}
\begin{equation}
\centering
\left \| \epsilon_{\theta}(\mathrm {E}[\mathbf{x}^{gen}_{d,t}],\mathbf{c}_{d},t)-\epsilon_{\theta}(\mathbf{x}^{true}_{d,t},\mathbf{c}_{d},t) \right \|^{2}
\label{eq:3}
\end{equation}
where $\mathbf{x}^{gen}_{d,t}$ and $\mathbf{x}^{true}_{d,t}$ shall be perturbed by the same noise at arbitrary diffusion step $t$. And we can substitute $\mathrm {E}[\mathbf{x}^{gen}_{d}]$ by the mean value of $B$ randomly generated samples:
\begin{equation}
\centering
\mathrm {E}[\mathbf{x}^{gen}_{d,t}]=\frac{1}{B}\sum_{i=1}^{B}\mathbf{x}^{gen,i}_{d,t}
\label{eq:4}
\end{equation}
Besides, we can conduct some experiments to further determine whether we should append the prior preservation loss in \eqref{eq:3} as~\cite{Ruiz_2023_CVPR}. 

\textcolor{blue}{Q1: How to condition the forecast distribution on past charging load and complementary covariates?} \\
(1) in the field of probabilistic time-series forecasting, simply \textcolor{green}{concatenate} $\mathbf{x}_{t}$ and $\mathbf{c}_{t}$ into multi-dimensional input vector for single RNN unit or \textcolor{green}{latent embedding fusion} in time imputation CSDI~\cite{NEURIPS2021_cfe8504b}.
(2) in the scope of text-to-image generation, classifier-based guided \& classifier-free guided \& \textcolor{green}{cross-attention mechanism} in each U-Net layer, due to a consensus in multi-modal representation that paired texts and images should own aligned latent semantics. Nevertheless, we do not require the high-level features of predicted profiles and input conditional terms shall be aligned, we instead anticipate the profiles of future outcomes should comply to the actually observed fact $\mathbf{c}_{t}$. \textcolor{green}{AdaGN}~\cite{NEURIPS2021_49ad23d1}.

\textcolor{blue}{Q2: How to incorporate conditional variables into our denoising diffusion model?} \\
see proposal 1.

Previous works focus on setting up EV and energy storage models with known parameters~\cite{pozo2022linear}.

\textcolor{blue}{Q1: Why EV charging load forecast is essential?} \\
(1) proliferate EV integration, stochastic and volatile charging load, operating stability/security of distribution grid and EVCS, promote EV infrastructure utility, optimally operate distribution grid with EVCS. \\
(2) applications: coordinated dispatch of EV and renewables~\cite{9055130}, optimal charging scheduling~\cite{8521585}, demand-response (V2G, controlled charging, provide ancillary services like frequency regulation, peak load curtailment)~\cite{BUZNA2021116337}, day-ahead market bidding, energy management in microgrid~\cite{JALALI2022108351}.

\textcolor{blue}{Q2: Why probabilistic not deterministic?} \\
(1) another perspective of appreciating the stochasticity and uncertainty of EV charging load, i.e., predictive distribution estimation, in contrast to DiffCharge. \\
(2) point forecast is unreliable due to the tremendous randomness of charging behaviors, model forecast uncertainties, reliable charging decision making, risk management, robust scheduling, stochastic optimization \\
(3) participate in VPP, minimize operational and energy deviation costs resulting from EV demand forecast uncertainties~\cite{10121507}.

\textcolor{blue}{Q3: Why do we focus on directly model the joint (conditional) predictive distribution instead of other methods, including quantile regression, PI construction, probabilistic auto-regression?} \\
(1) generate much larger number of possible outcomes to consititute a more accurate and reliable PI. \\
(2) non-autoregressive (joint and global manner), get rid of the reliance on RNN, better capture the complex temporal correlations.

\textcolor{blue}{Q4: What is difference between our diffusion-based conditional distribution approximation with other explicit forecasting distribution modeling? In addition, What is the difference between the problem setup of EV-PLF and other typical load PLF?} \\
(1) use conditional terms $\mathbf{c}_{d}$ to constrain, explain why temperature (battery dynamic properties and EV travelling modes) and EV number (charging amount), instead of typical known covariates $\mathbf{c}_{d-N:d}$. \\
(2) short-term forecast (day-ahead), not real-time (very-short) prediction, min-head or hourly. \\
(3) joint distribution, non-autoregressive paradigm.
(4) none statistical assumption, i.e. distributional form.

\textcolor{red}{Task for Yize: Mention more on charging mode, charging characteristics: check paper High-Voltage Stations for Electric Vehicle Fast-Charging: Trends, Standards, Charging Modes and Comparison of Unity Power-Factor Rectifiers}

\textcolor{blue}{scaling technique, knowledge evnum up then load up}
